PriPrune: Quantifying and Preserving Privacy in Pruned Federated Learning

Federated learning (FL) is a paradigm that allows several client devices and a server to collaboratively train a global model, by exchanging only model updates, without the devices sharing their local training data. These devices are often constrained in terms of communication and computation resources, and can further benefit from model pruning -- a paradigm that is widely used to reduce the size and complexity of models. Intuitively, by making local models coarser, pruning is expected to also provide some protection against privacy attacks in the context of FL. However this protection has not been previously characterized, formally or experimentally, and it is unclear if it is sufficient against state-of-the-art attacks. In this paper, we perform the first investigation of privacy guarantees for model pruning in FL. We derive information-theoretic upper bounds on the amount of information leaked by pruned FL models. We complement and validate these theoretical findings, with comprehensive experiments that involve state-of-the-art privacy attacks, on several state-of-the-art FL pruning schemes, using benchmark datasets. This evaluation provides valuable insights into the choices and parameters that can affect the privacy protection provided by pruning. Based on these insights, we introduce PriPrune -- a privacy-aware algorithm for local model pruning, which uses a personalized per-client defense mask and adapts the defense pruning rate so as to jointly optimize privacy and model performance. PriPrune is universal in that can be applied after any pruned FL scheme on the client, without modification, and protects against any inversion attack by the server. Our empirical evaluation demonstrates that PriPrune significantly improves the privacy-accuracy tradeoff compared to state-of-the-art pruned FL schemes that do not take privacy into account.

==> background.tex <==
We start by
\subsection{Federated Learning Setting}
Consider an FL system involving $N$ clients participating in the training task. Client $i$ has the local dataset $\mathcal{D}_{i}$ with $\left | \mathcal{D}_{i} \right  |$ samples, drawn from non-independent and non-identically (Non-IID) distribution $\mathcal{X}_{i} (\mu_{i},\,\sigma_{i}^{2})$.

The goal of using FL is to learn a global model $F$  for the (aggregation) server.
Given the loss function $\ell(\bm{w};\mathcal{D})$,
the objective function of FL can be described as
$$\mathcal{L}(\bm{w}) = \mathbb{E}_{\mathcal{D}\sim \mathcal{X}}\left[\ell({\bm{w};\mathcal{D}}) \right]$$
Therefore, the task becomes:
$$ \bm{w}^{*} = \mathop{\arg\min}_{\bm{w} \in \mathds{R}^{d}} \mathcal{L}(\bm{w})$$
To find the optimal $\bm{w}^{*}$, Stochastic Gradient Descent (SGD) is employed to optimize the objective function. 

Let $T$ be the total number of communications. The FL model training process entails several rounds of communication between clients and the server. The global model $F$ is first initialized at a random state and, then, in round $t$ the following steps are taken:
\begin{enumerate}
    \item \textbf{Broadcast}:
The server first randomly selects a subset of clients $\mathcal{S}^{t}$ ($\left | \mathcal{S}^{t} \right | = \mathcal{C} \geq 1$) and then distributes the latest global model to all chosen clients.
    \item \textbf{Local Training}: The selected client $i$ performs local computation based on the global model and its local dataset $\mathcal{D}_i$ and sends the update $\bm{w}_i^t$ back to the server:
    $$\bm{w}_{i}^{t} \leftarrow  \bm{w}_{i}^{t-1} - r\frac{\partial \ell_{i}({\bm{w}_{i}^{t-1};\mathcal{D}_{i}})}{\partial \bm{w}}$$
    where $r$ is the learning rate.
    \item \textbf{Aggregation} By applying an aggregation rule to all these updates, the server updates the global model $F$, and the process repeats.
\end{enumerate}

\subsection{Model Pruning}
Model pruning is one of the promising methods to enable heterogeneous neural networks by eliminating unnecessary weights from neural networks and thus bringing reduction to the computation costs as well as privacy leakage. Most of the work requires two phrases:
\begin{enumerate}
    \item \textbf{Pre-training Phase}: Randomly initialize a neural network and train the network to obtain a model $F({\bm{w};\mathcal{D}})$.
    \item \textbf{Pruning Phase} Taking the pre-trained model $F({\bm{w};\mathcal{D}})$ as input, the pruning process generates a new model $f({\bm{w} \odot m ;\mathcal{D}})$, where $m\in \left \{0, 1 \right \}^{|\bm{w}|}$ is a binary mask to denote certain parameters $\bm{w}$ to be set to zero with the pruning rate $p$ and  $\odot$ denotes Hadamard product. The pruning mask $m$ is computed from a certain pruning policy $\mathds{P}$.
\end{enumerate}


